Lessons learned from the early performance evaluation of Intel Optane DC Persistent Memory in DBMS

Non-volatile memory (NVM) is an emerging technology, which has the persistence characteristics of large capacity storage devices(e.g., HDDs and SSDs), while providing the low access latency and byte-addressablity of traditional DRAM memory. This unique combination of features open up several new design considerations when building database management systems (DBMSs), such as replacing DRAM (as the main working space memory) or block devices (as the persistent storage), or complementing both at the same time for several DBMS components (such as access methods,storage engine, buffer management, logging/recovery, etc). However, interacting with NVM requires changes to application software to best use the device (e.g. mmap and clflush of small cache lines instead of write and fsync of large page buffers). Before introducing (potentially major) code changes to the DBMS for NVM, developers need a clear understanding of NVM performance in various conditions to help make better design choices. In this paper, we provide extensive performance evaluations conducted with a recently released NVM device, Intel Optane DC Persistent Memory (PMem), under different configurations with several micro-benchmark tools. Further, we evaluate OLTP and OLAP database workloads (i.e., TPC-C and TPC-H) with Microsoft SQL Server 2019 when using the NVM device as an in-memory buffer pool or persistent storage. From the lessons learned we share some recommendations for future DBMS design with PMem, e.g.simple hardware or software changes are not enough for the best use of PMem in DBMSs.

==> Makefile <==
DOC_ROOT_NAME := sig-alternate-sample
DOC_ROOT_TEX := $(DOC_ROOT_NAME).tex
DOC_ROOT_BIB := sigproc.bib
DOC_ROOT_AUX := $(DOC_ROOT_NAME).aux
DOC_ROOT_BBL := $(DOC_ROOT_NAME).bbl
DOC_ROOT_PDF := $(DOC_ROOT_NAME).pdf

# Rebuild if any of these files have changed.
DEPS := $(DOC_ROOT_TEX) \
    $(DOC_ROOT_BIB) \
    Sections/*.tex \
    Figures/*

.PHONY: all
all: $(DOC_ROOT_PDF)

# The first pdflatex is to refresh the $(DOC_ROOT_AUX) file for the
# $(DOC_ROOT_BBL) to use during the bibtex run.
# The final pdflatex command is to make sure any addition changes to
# $(DOC_ROOT_AUX) are incorporated.
# Note our current project makes no use of \index directives, so we don't call
# makeindex at the moment.
$(DOC_ROOT_PDF): $(DEPS)
	pdflatex $(DOC_ROOT_TEX)
	bibtex $(DOC_ROOT_NAME)
	pdflatex $(DOC_ROOT_TEX)
	pdflatex $(DOC_ROOT_TEX)

.PHONY: clean
clean:
	rm -f $(DOC_ROOT_PDF)
	rm -f $(DOC_ROOT_AUX)
	rm -f $(DOC_ROOT_BBL)
	rm -f $(DOC_ROOT_NAME).log
	rm -f $(DOC_ROOT_NAME).blg
	rm -f Sections/*.log


==> Sections/five-minute_rule.tex <==
\section{Performance-cost trade-offs analysis}\label{sec: five-min-rule}

+\cmt{Be consistent in your capitalization - it should be "The Five Minute Rule" or "The 5 Minute Rule" (the original) throughout the document}

This section will focus on the performance-cost trade-offs discussion for \nvm\ in various configurations by referencing the performance characteristics in Section \ref{sec: device_character}. Same as Section \ref{sec: device_character}, both the cases when \nvm\ is configured as persistent storage and system memory will be discussed as below.

\subsection{\nvm\ as persistent storage}\label{sec: performance_cost_storage}
\subsubsection{what is \fiveminrule}
In this subsection, we will use classical \fiveminrule\ to compare the performance per dollar expense between different configurations of \nvm\ and \ssd. \fiveminrule\ was firstly introduced by Jim gray and Franco Putzolu in 1987 \cite{gray19875} and revisited three times in 1997 \cite{gray1997five}, 2007 \cite{graefe2007five} and 2017 \cite{appuswamy2017five} respectively, which requires the evaluations of {\em break-even interval}. A data page should be cached in DRAM as long as its two continuous access is within the break-even interval, which is evaluated with the following formula:
\cmt{Later you reference this as "Equation" 1, but the term "Equation" doesn't appear next to the formula}
\begin{equation}\label{eq: five-min-rule}
\frac{PagesPerMBofDRAM}{AccessPerSecondPerDisk}\times \frac{PricePerDiskDrive}{PricePerMBofDRAM}
\end{equation}

\cmt{introduce the meaning of five minute rule and its change with the hardware price change and performance change}
where the two ratio are termed as \textit{technology ratio} and \textit{economic ratio} respectively and \\ $AccessPerSecondPerDisk$ typically represents the random access (read or write) IOPS, which will be the inverse of the latency under the latency-sensitive workloads, In what follows, the evaluations will be based on the latency of random read or random write and the evaluation over IOPS will be left for future work.
%When 
% which was 30 accesses/second one disk with two disk channels when 
% the five-minute rule was firstly proposed in 1987 \cite{gray19875}
% . At that point, the disk price was 15k\$ and the unit memory price was 5\$/KB. By plugging those values into Equation \ref{eq: five-min-rule}
%, the break-even interval was 400 seconds with I/O size 1KB, which is around 5 minutes. The authors of \cite{gray1997five} also extended the evaluations of this rule for sequential read workloads and proposed one-minute sequential rule with large I/O size (e.g. 64 KB). Intuitively speaking, given the same workloads and the storage devices worth the same amount of money (e.g. multiple cheaper devices VS one more expensive devices), 
Intuitively speaking, between two different storage devices, the smaller the break-even interval is, the less amount of data should be cached within the memory to achieve the same performance, thereby saving the cost on buying memory. 
%, which can provide instructions on the data placement problem in some typical query process algorithms where sequential access occurs, such as sort, join, cube, etc.

\cmt{All occurences of "NVME" should really be "NVMe"}
\cmt{I would also write "Pmem" as "PMem"}
\cmt{Perhaps use \\pmem aliases as you did in some places for other terms (but be consistent in their usage, else they don't help much)}

\cmt{talk about pmem and ins influence for five-minute rule}
%Since its propose in 1987, the break-even interval value has been constantly changed with the emerging new hardware technologies, especially with the use of SSDs \cite{graefe2007five, appuswamy2017five}. The trend of hardware changes continues in recent years, which includes
%which results in the decrease of the hardware prices and improved throughput. But the changes over  \textit{technology ratio} and \textit{economic ratio} were different due to the quicker price drop for DRAM compared to disks and the reduced I/O overhead, which pushes the break-even values from around 5 minutes to hours (as reported in \cite{graefe2007five} and \cite{appuswamy2017five}) and requires almost all the data to reside in DRAM. 
%At the same time, more new persistent storage devices (e.g. SSD) have been introduced, which can thus serve as intermediate storage layer because of their cheaper price compared to DRAM and better I/O performance relative to disks. It has been shown that with SSD as the storage in the system, five-minute rule still roughly holds in typical I/O size\cite{graefe2007five, appuswamy2017five}.
%the inventions of more advanced SSDs (e.g. \ssd) and \nvm. As shown in Section  \ref{sec: micro_res}, \nvm\ significantly boosts the throughput compared to SSDs, which drives us to re-evaluate the break-even interval with their specific performance characteristics and prices. In terms of \nvm, its various configurations and I/O scenarios incur additional complexity for the break-even interval analysis. In what follows, the break-even interval values are calculated with two interleaved \nvm s with various I/O sizes (64 B - 64 KB) and all the I/O scenarios discussed in Section \ref{sec: micro_res}, which includes \daxio\ and \fileio\ in \fsdax\ mode and \fileio\ in \sector\ mode with both random read and sequential read workloads. The baseline case is that the \fileio\ is issued against \ssd\ with DRAM as system memory. According to Section \ref{sec: micro_res}, random read and sequential read in \nvm\ have very similar performance patterns across different I/O scenarios. So we expect that the they should also have similar evaluation results and thus only the results under random read workloads are reported to save space.
%On the other hand, when \nvm\ is configured as memory mode, \ssd\ is the persistent storage. 



To compare the trade-off intervals of \nvm\ and \ssd, the price information is essential. Currently, the unit price of 16 GB DDR4 DRAM is about \$6.25/GB \footnote{https://memory.net/memory-prices/} while the unit price of \ssd\ price is \$0.220 per GB \footnote{https://www.intel.com/content/www/us/en/products/memory-storage/solid-state-drives/data-center-ssds/d7-series/dc-p4510-series/dc-p4510-4tb-2-5inch-3d2.html}. But unfortunately, the price of \nvm\ is not available in the official website\footnote{https://www.intel.com/content/www/us/en/products/memory-storage/optane-dc-persistent-memory/optane-dc-512gb-persistent-memory-module.html} although we assumed that the unit price of \nvm\ should be lower than the unit price of DRAM but higher than that of \ssd. So in what follows, first of all, the evaluations of the break-even intervals depend on a fixed \nvm\ unit price, \$6.25/GB, which is the highest unit price in our assumed price range. For fair comparison, the capacity of \ssd\ is assumed to be same as \nvm\ in one socket, i.e. 1TB. After that, we explored in which price range, \nvm\ has smaller break-even interval than \ssd\ for different I/O sizes.





%provide instructions on in which price range, .


%However, we can expect that the unit price of \nvm\ should lie between the DRAM unit price and \ssd\ unit price. Currently, the 16 GB DDR4 DRAM price is about \$100 \footnote{https://memory.net/memory-prices/}, i.e. \$6.25 per GB while the 4TB \ssd\ price is \$784, i.e. \$0.196 per GB. So the reasonable unit price for \nvm\ would be \$0.196-\$6.25 per GB. In what follows, our assumed prices for \nvm\ include the prices in that price interval, i.e. \$2 per GB (low price), \$5 per GB (intermediate price). But we also consider a relative higher price, i.e.\$10 per GB to reflect its higher cost in the early stage since the first release of \nvm. Given the (assumed) price information above and the performance measurements .


%Introduce the price details of the device, assume the unit price of pmem lies between DRAM and NVME SSD:
%DDR4 DRAM price: about 100 for 16GB (), NVME SSD price: about 784 for 4T (), we can assume that the PMEM price is (\$ 2.5 per GB), which is 2560 for 1024GB.



%Then we can give the \textit{economic ratio} for those different configurations, which only depends on the device type.

%\begin{table}
%\begin{center}
%\begin{tabular}{|c|c|}\hline
%configurations&economic ratio\\\hline
%\nvm & 409600 \\\hline
%\ssd & 125440\\\hline
%\end{tabular}
%\caption{Five-minute rule economic ratios}
%\end{center}
%\end{table}


%\newcommand{\puredax}{\nvm\ fsdax mode direct IO}
%\newcommand{\daxfio}{\nvm\ fsdax mode file IO}
%\newcommand{\stfio}{\nvm\ sector mode file IO}
%\newcommand{\ssdfio}{\ssd\ file IO}

%\begin{table*}[h]
%\centering
%\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}\hline
%Page size&256 B&512 B & 1KB & 2KB & 4KB & 8KB& 16KB & 32KB& 64KB\\\hline
%\makecell{\nvm\ fsdax \\ mode direct IO} & 347.86 & 181.24 & 171.38&  98.94& 63.60 & 51.46& 45.47 &41.83& 41.03 \\\hline
%\makecell{\nvm\ fsdax \\ mode file IO}\ & 660.64& 375.78& 198.83& 102.91& 58.51& 46.97& 42.74& 41.16& 40.51\\ \hline
%\makecell{\nvm\ sector\\ mode file IO} & 1122.19 & 553.51& 274.90& 136.53&68.27& 48.30& 44.60 & 41.56&34.41\\ \hline
%\makecell{\ssd\ \\ file IO} & 1960.00& 983.84&501.76& 246.93&       125.94& 84.30&60.78&53.00&39.76\\ \hline
%\end{tabular}
%\caption{Five-minute rule break-even intervals (random read non-direct IOs) with IOPS values}\label{table: 5-min-rule-rr-iops-non-direct-io}
%\end{table*}

%\begin{figure}[h]
%    \centering
%    \includegraphics[width=0.5\textwidth, height=0.2\textwidth]{figures/break_even_interval.png}
%    \caption{Break-even values with random read access (\$6.25/GB, IOPS)}    
%    \label{fig:five-min_rr_2}
%\end{figure}


\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth, height=0.2\textwidth]{figures/break_even_interval_lat.png}
    \caption{Break-even values with random read access (\$6.25/GB, latency)}    
    \label{fig:five-min_rr_lat}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth, height=0.2\textwidth]{figures/break_even_interval_lat_rw.png}
    \caption{Break-even values with random write access (\$6.25/GB, latency)}    
    \label{fig:five-min_rw_lat}
\end{figure}

%\begin{figure}[h]
%    \centering
%    \includegraphics[width=0.4\textwidth, height=0.2\textwidth]{figures/five-min_rule_rr_10.png}
%    \caption{Break-even values with random read access (\$10/GB)}    
%    \label{fig:five-min_rr_10}
%\end{figure}

\cmt{the following two figures side by side}

%\begin{figure}
%\centering
%\begin{subfigure}{.2\textwidth}
%  \centering
%  \includegraphics[width=1\textwidth, height=1\textwidth]{figures/break_even_interval_change_512b.png}
%\caption{I/O size = 512 Bytes}    
%    \label{fig:five-min_rr_price_change_512b}
%\end{subfigure}%
%\begin{subfigure}{.2\textwidth}
%  \centering
%      \includegraphics[width=1\textwidth, height=1\textwidth]{figures/break_even_interval_change_8k.png}
%\caption{I/O size = 4 K}    
%    \label{fig:five-min_rr_price_change_8k}
%    \end{subfigure}
%\caption{Break-even values change with varied \nvm\ price}
%\label{fig:test}
%\end{figure}
%Break-even values change with varied \nvm\ price (I/O = 8 KB)

%
%\begin{figure}[h]
%    \centering
%    \includegraphics[width=0.3\textwidth, height=0.25\textwidth]{figures/break_even_interval_change_512b.png}
%    \caption{Break-even values change with varied \nvm\ price (I/O = 512 Bytes)}    
%    \label{fig:five-min_rr_price_change_512b}
%\end{figure}

%\begin{figure}[h]
%    \centering
%    \includegraphics[width=0.3\textwidth, height=0.2\textwidth]{figures/break_even_interval_change_8k.png}
%    \caption{Break-even values change with varied \nvm\ price (I/O = 8 KB)}    
%    \label{fig:five-min_rr_price_change_8k}
%\end{figure}


%\begin{table*}[h]
%\small
%\centering
%\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}\hline
%Page size&64B&128B&256 B&512 B & 1KB & 2KB & 4KB & 8KB& 16KB & 32KB& 64KB\\\hline
%\makecell{\nvm\ fsdax \\ \daxio\ (\$2/GB)}&144.03&100.26  &39.46&42.44&78.97&52.5&39.38&34.55&34.68&34.84& 33.82 \\\hline
%\makecell{\nvm\ fsdax \\ \fileio\ (\$2/GB)} &3459.85&1728.55&871.25&425.24&202.62&97.88&56.04&40.97&35.32
%&34.05&33.4 \\ \hline
%\makecell{\nvm\ sector\\ \fileio\ (\$2/GB)} &-&-&-&-&-&-&49.92&40.96&37.75&36.87&36.43\\ \hline
%%\makecell{\nvm\ fsdax \\ \daxio\ \\ (\$5/GB)}&360.07&250.65& 98.66&106.11&197.42&131.24&98.46&86.38&86.7&87.09&84.56 \\\hline
%%\makecell{\nvm\ fsdax \\ \fileio\ \\ (\$5/GB)} &8649.62&4321.37 &2178.12&1063.1&506.55&244.69&140.11&102.43&88.31&85.12& 83.5\\ \hline
%%\makecell{\nvm\ sector\\ \fileio\ \\ (\$5/GB)} &-&-&-&-&-&-&124.79&102.41&94.38&92.17&91.07\\ \hline
%\makecell{\nvm\ fsdax \\ \daxio\ (\$10/GB)}&720.13&501.30&197.32&212.22&394.84&262.48&196.92&172.76&173.39&174.18&169.12
%\\\hline
%\makecell{\nvm\ fsdax \\ \fileio\ (\$10/GB)} &17299.23&8642.74&4356.24&2126.20&1013.11&489.38&280.22&204.85&176.62&170.23&167.00
%\\ \hline
%\makecell{\nvm\ sector\\ \fileio\ (\$10/GB)} &-&-&-&-&-&-&249.58&204.81&188.76&184.34&182.14\\ \hline
%\makecell{\ssd} &-&-&-&631.39&314.6&157.09&79.38  &62.75&52.83&51.93&50.85\\ \hline
%\makecell{\nvm\ -\ssd\ \\ (\$2/GB)}&-&-&-&1973.11&983.13&490.90&248.06&196.10&165.09&162.28&158.91\\ \hline
%%\makecell{\nvm\ -\ssd\ \\ (\$5/GB)}&-&-&-&789.24&393.25&196.36&99.22&78.44&66.03&64.91&63.57\\ \hline
%\makecell{\nvm\ -\ssd\ \\ (\$10/GB)}&-&-&-&394.62&196.63&98.18&49.61&39.22&33.02&32.46&31.78
%\\\hline
%\end{tabular}
%\caption{Five-minute rule break-even intervals (s) with random read I/O}\label{table: 5-min-rule-rr-iops}
%\end{table*}



%\begin{table}[h]
%\small
%\centering
%\begin{tabular}{|c|c|c|c|c|c|c|c|c|}\hline
%I/O size&512 B & 1KB & 2KB & 4KB & 8KB& 16KB & 32KB& 64KB\\\hline
%\makecell{random \\ read}&29.75&7.97&5.98&4.03&3.63&3.05&2.98&3.01\\\hline
%\makecell{sequential \\ read}&42.31&19.67&9.61&4.60&3.78&3.18&3.27&3.15\\ \hline
%\end{tabular}
%\caption{\nvm\ unit price threshold (\$)}\label{table: price-threshold}
%\end{table}





%\begin{table*}[h]
%\centering
%\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}\hline
%I/O size&256 B&512 B & 1KB & 2KB & 4KB & 8KB& 16KB & 32KB& 64KB\\\hline
%\makecell{\nvm\ \fsdax\ \daxio} &715.98&544.77&332.60&218.93&149.09&123.75&113.66&105.11,&106.48
%\\ \hline
%%\makecell{\nvm\ fsdax \\ mode direct IO} & 786.43&586.55&334.64&233.47&157.70&133.12&119.81&112.90     &110.08 \\\hline
%\makecell{\nvm\ \fsdax\ \fileio}\ & 3915.78&2056.19&1167.36&663.55&379.90& 244.22&182.27&149.76&136.32\\ \hline
%\makecell{\nvm\ \sector\ \fileio} & -& -&-&-&1781.76&1224.70&944.13&808.96&737.28\\ \hline
%\makecell{\ssd} &- &21600.77&10456.68&5204.51&2662.15&1453.38&889.68&594.04&424.83\\ \hline
%\makecell{\nvm\ -\ssd}&-&21771.37&10239.67&5228.34&2665.91& 1449.15&885.76&587.18&414.15 \\\hline
%\end{tabular}
%\caption{Five-minute rule break-even intervals (random read direct IO) with latency}\label{table: 5-min-rule-rr-latency}
%\end{table*}






%
%\begin{table*}[h]
%\centering
%\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}\hline
%Page size&256 B&512 B & 1KB & 2KB & 4KB & 8KB& 16KB & 32KB& 64KB\\\hline
%\makecell{\nvm\ fsdax \\ mode direct IO} &46.41&43.81& 45.51&44.14& 42.31& 40.96& 40.44& 40.00& 39.75\\\hline
%\makecell{\nvm\ fsdax \\ mode file IO}\ &803.14& 388.25&181.24&94.81& 51.46& 41.63& 40.76& 40.38& 40.00 \\ \hline
%\makecell{\nvm\ sector\\ mode file IO} & 769.20& 431.16&214.45&116.36& 64.81& 46.13& 45.63& 45.71& 45.71\\ \hline
%\makecell{\ssd\ \\ file IO} & 910.22& 409.60& 260.89& 165.16& 160.75& 157.54 & 161.01&167.32& 152.38\\ \hline
%\end{tabular}
%\caption{Five-minute rule break-even intervals (sequential read) with latency}\label{table: 5-min-rule-sr}
%\end{table*}


%\begin{table*}[h]
%\centering
%\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}\hline
%Page size&256 B&512 B & 1KB & 2KB & 4KB & 8KB& 16KB & 32KB& 64KB\\\hline
%\makecell{\nvm\ fsdax \\ mode direct IO} &46.41&43.81& 45.51&44.14& 42.31& 40.96& 40.44& 40.00& 39.75\\\hline
%\makecell{\nvm\ fsdax \\ mode file IO}\ &803.14& 388.25&181.24&94.81& 51.46& 41.63& 40.76& 40.38& 40.00 \\ \hline
%\makecell{\nvm\ sector\\ mode file IO} & 769.20& 431.16&214.45&116.36& 64.81& 46.13& 45.63& 45.71& 45.71\\ \hline
%\makecell{\ssd\ \\ file IO} & 278.76 & 125.44& 79.90& 50.58& 49.23&48.25 & 49.31&51.24&46.67\\ \hline
%
%\end{tabular}
%\caption{Five-minute rule break-even intervals (sequential read non-direct IO) with bandwidth}\label{table: 5-min-rule-sr-non-direct-io}
%\end{table*}


%\begin{table*}[h]
%\centering
%\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}\hline
%I/O size&64B&128B&256 B&512 B & 1KB & 2KB & 4KB & 8KB& 16KB & 32KB& 64KB\\\hline
%\makecell{\nvm\ \fsdax\ \\ \daxio\ (\$2/GB)} &40.03&36.75&33.99&33.15&34.5&34.69&34.65&33.44&33.3 &33.83&33.37\\\hline
%\makecell{\nvm\ \fsdax\ \\ \fileio\ (\$2/GB)}\ &2927.35&1462.89&743.01&390.14&178.82&95.27&54.51&37.26& 33.9&33.35&33.03 \\ \hline
%\makecell{\nvm\ \sector\ \\ \fileio (\$2/GB)} &-&-&-& -&-&-&51.58&38.2&36.89&37.19&37.42\\ \hline
%%\makecell{\nvm\ fsdax \\ \daxio\ (\$5/GB)} &100.06&91.88& 84.98&82.87&86.24&86.73&86.62&83.6&83.24&84.58&83.42\\\hline
%%\makecell{\nvm\ fsdax \\ \fileio\ (\$5/GB)} &7318.37 &3657.24&1857.52&975.36&447.05&238.18&136.27&93.14&84.74&  83.37&82.56\\ \hline
%%\makecell{\nvm\ sector\\ \fileio (\$5/GB)} &-&-&-& -&-&-&128.94&95.51&92.22&92.97&93.55\\ \hline
%\makecell{\nvm\ \fsdax\ \\ \daxio\ (\$10/GB)} &200.13&183.76&169.96&165.74&172.48&173.46&173.24&167.21&166.48&169.16&166.83
%\\\hline
%\makecell{\nvm\ \fsdax\ \\ \fileio\ (\$10/GB)} &14636.74&7314.47&3715.04&1950.72&894.09&476.36&272.55&186.28&169.48&166.74&165.13
%\\ \hline
%%\makecell{\nvm\ sector\\ \fileio (\$10/GB)} &-&-&-& -&-&-&257.89&191.02&184.43&185.94&187.11\\ \hline
%\makecell{\ssd} &-&-&-&701.22&339.32&166.78& 79.61&63.26&52.98&55.28&52.62\\ \hline
%\makecell{\nvm\ -\ssd\ \\ (\$2/GB)} &-&-&-&2191.32&1060.37&521.19&248.79&197.67&165.57&172.73&164.45
%\\ \hline
%%\makecell{\nvm\ -\ssd\ \\ (\$5/GB)} &-&-&-&876.53&424.15&208.47&99.52&79.07&66.23&69.09&65.78
%%\\ \hline
%\makecell{\nvm\ -\ssd\ \\ (\$10/GB)} &-&-&-&438.26&212.07&104.24&49.76&39.53&33.11&34.55&32.89
%\\ \hline
%\end{tabular}
%\caption{Five-minute rule break-even intervals (seconds) with sequential read I/O}\label{table: 5-min-rule-sr-direct-io}
%\end{table*}


%\begin{table*}[h]
%\centering
%\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}\hline
%I/O size&256 B&512 B & 1KB & 2KB & 4KB & 8KB& 16KB & 32KB& 64KB\\\hline
%\makecell{\nvm\ fsdax \\ mode direct IO} &46.41&43.81& 45.51&44.14& 42.31& 40.96& 40.44& 40.00& 39.75\\\hline
%\makecell{\nvm\ fsdax \\ mode file IO}\ &803.14& 388.25&181.24&94.81& 51.46& 41.63& 40.76& 40.38& 40.00 \\ \hline
%\makecell{\nvm\ sector\\ mode file IO} & 769.20& 431.16&214.45&116.36& 64.81& 46.13& 45.63& 45.71& 45.71\\ \hline
%\makecell{\ssd\ \\ file IO} & 278.76 & 125.44& 79.90& 50.58& 49.23&48.25 & 49.31&51.24&46.67\\ \hline
%\end{tabular}
%\caption{Page utility for B-tree nodes on disk}\label{table: index-page-size-rr-non-direct-io}
%\end{table*}






%\begin{table*}[h]
%\small
%\centering
%\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}\hline
%I/O size&256 B&512 B & 1KB & 2KB & 4KB & 8KB& 16KB & 32KB& 64KB\\\hline
%\makecell{\nvm\ fsdax \\ mode direct IO} & 151.70& 132.99& 131.28& 128.81&133.33&115.06 & 115.84 & 114.29 & 113.48\\\hline
%\makecell{\nvm\ fsdax \\ mode file IO}& 1476.03& 738.01& 372.36& 186.18& 251.60& 262.56& 272.92& 274.68& 278.26\\ \hline
%\makecell{\nvm\ sector\\ mode file IO} \\ \hline
%\makecell{\ssd\ \\ file IO} \\ \hline
%\end{tabular}
%\caption{Five-minute rule break-even intervals (random write)}
%\end{table*}


%calculate the break-even values in different configurations, DRAM-SSD, DRAM-storage mode, DRAM-fsdax file IO, DRAM-fsdax direct IO, memory mode-nvme SSD

\cmt{whether to put those values in the graph}

\begin{table}
\small
\begin{center}
\begin{tabular}{|c|c|c|c|}\hline
SSD type& latency ($\mu$s) & price & \makecell{break-even \\ interval (seconds)} \\\hline
\makecell{INTEL SSD \\DC P4501 \\ SERIES (1TB)} & 100 (r)/ 30(w) & \$ 479.5 & 1918 (r)/ 575.4 (w) \\\hline
\makecell{INTEL SSD  \\ DC P4500 \\ SERIES (1TB)}& 85(r)/ 20(w) & \$ 385 & 1309 (r)/308 (w) \\\hline
\makecell{INTEL SSD  \\ DC D3600 \\ SERIES (1TB)}& 30(r)/ 30(w) & \$ 1200 & 1440 (r)/1440 (w)\\\hline
\end{tabular}
\caption{Specifications of other SSDs}\label{table: SSD_spec}
\end{center}
\end{table}




\begin{table}
\small
\begin{center}
\begin{tabular}{|c|c|}\hline
SSD type& \makecell{cross-over \nvm\ unit price}\\\hline
\makecell{\ssd\ (I/O = 512B)} &  19.49(r)/5.12 (w)\\ \hline
\makecell{\ssd\ (I/O = 4K)} & 10.66(r)/1.05(w)\\ \hline
\makecell{INTEL SSD DC P4501 \\ SERIES (1TB, I/O = 4K)} & 28.58(r)/4.86(w)\\\hline
\makecell{INTEL SSD DC P4500 \\ SERIES (1TB, I/O = 4K)} & 19.50(r)/2.6(w)\\\hline
\makecell{INTEL SSD DC D3600 \\ SERIES (1TB, I/O = 4K)} & 12.16(r)/12.16(w)\\\hline
\end{tabular}
\caption{cross-over unit price of \nvm\ compared to different SSDs}\label{table: cross_over_point}
\end{center}
\end{table}


\subsubsection{Break-even interval evaluation in \nvm}

\textbf{Fixed \nvm\ price} Given the fixed \nvm\ unit price (\$6.25/GB), the break-even intervals under varied I/O sizes are presented in Figure \ref{fig:five-min_rr_lat} and Figure \ref{fig:five-min_rw_lat} for random read workloads and random write workloads respectively. In terms of random read, with I/O sizes no more than the typical I/O sizes used in database systems (4KB or 8KB), \daxio\ over \nvm\ leads to smaller break-even interval than \ssd. Notice that the break-even interval of \nvm\ should be even smaller with cheaper \nvm, indicating that as long as the unit price of \nvm\ is less than that of DRAM and typical I/O size or smaller I/O size is used in DBMS, \nvm\ should have better performance-price trade-offs than \ssd. This result implies that under any read-dominated OLTP workloads over proper database configurations (e.g. default or even smaller page sizes), \daxio\ over \nvm\ should be preferred compared to \ssd.

However, due to the significant better write performance (compared to read) of \ssd, the performance gap between \nvm\ and \ssd\ becomes much smaller, leading to smaller break-even interval of \ssd\ than \nvm\ with all I/O sizes. But with the unit price smaller than the DRAM unit price, \nvm\ should have smaller break-even interval and thus there still exist an opportunity for \nvm\ to win, which drives us to explore below which unit price (called cross-over unit price), \nvm\ is better than \ssd.

%
%\begin{foo}
%\textit{With proper unit price, \nvm\ can have better performance per unit price than \ssd\ when \nvm\ is used as persistent storage.}
%\end{foo}

\textbf{Varied \nvm\ price} We present the results from two typical I/O sizes (512 Bytes and 4KB) in the first two rows of Table \ref{table: cross_over_point}. 4KB is the typical page sizes in many database systems such as SQL server, MySQL etc. while 512 Bytes is the minimal I/O size where \nvm\ and \ssd\ are comparable. The results show that the cross-over unit prices are \$ 5.12 and \$ 1.05 for the two I/O sizes respectively. It indicates that when the I/O size is small (e.g. 512 Bytes), as long as the unit price of \nvm\ is smaller than \$ 5.12, under any OLTP workloads (mixture of read and write), \nvm\ should be better. Notice that this cross-over unit price is pretty close to the DRAM unit price. As discussed in Section \ref{sec: micro_bench_storage}, once the extra overhead is excluded from FIO latency measurements with small I/O size, it is possible that the cross-over unit price is higher than the DRAM unit price. In contrast, with larger I/O size (4KB), the cross-over unit price is only \$ 1.05, relatively far away from the DRAM unit price, which indicates that once the \nvm\ becomes more expensive, under the write-intensive OLTP workloads with I/O size 4K, \ssd\ should be preferred. 


\begin{foo}
\textit{With smaller I/O size, \nvm\ with \fsdax\ \daxio\ can achieve better performance per unit price compared to \ssd. In contrast, \nvm\ will not have advantage in terms of performance per unit price compared to \ssd\ when the I/O size is large. }
\end{foo}

We also investigated other typical SSDs used in data center and calculated the break-even intervals in Table \ref{table: SSD_spec} based on the performance and price information collected from the device specification with I/O size 4K (shown in the same table). We also did similar comparison between \nvm\ and those SSDs and listed  the cross-over \nvm\ unit price in Table \ref{table: cross_over_point}, which shows higher value than DRAM unit price for random read. Similar to \ssd, it implies the benefit of \nvm\ \daxio\ over \ssd\ under read-dominated OLTP workloads. In terms of random writes, except the last SSD, \nvm\ can only be advantageous over the other SSDs with the unit price lower than DRAM unit price. But it can be expected that those cross-over \nvm\ unit price for random writes should be higher (possibly close or even exceed DRAM unit price) with smaller I/O sizes, in which cases, \nvm\ can be better than those SSDs even with slightly cheaper unit price relative to DRAM under any read-write mixed OLTP workloads.


\cmt{Comparison across varied I/O sizes}




%the break-even interval values under varied I/O scenarios (\daxio\ in \fsdax\ mode and \fileio\ in \fsdax\ mode, \sector\ mode and \ssd) with varied I/O sizes for random read I/Os are shown in Figure \ref{fig:five-min_rr_2}. 
%Also, due to the similar random read performance between \fileio\ in \fsdax\ mode and \fileio\ in \sector\ mode over \nvm\ (as shown in Section \ref{sec: micro_res}), their break-even interval values should be also very close. So only  one of them (i.e. the one for \fileio\ in \fsdax\ mode) is presented in Figure \ref{fig:five-min_rr_2} and Figure \ref{fig:five-min_rr_10}. 
%First of all, we observe that for \nvm, when the I/O size is small (e.g. 512 Bytes), the \daxio\ in \fsdax\ mode have the least break-even interval values compared to \fileio\ in \fsdax\ mode and \ssd, which is due to the relatively larger \textit{technology ratio} caused by the huge bandwidth gains of \daxio\ with small I/O size (e.g. the gain is 9.88 and 48.33 compared to \fileio\ in \fsdax\ mode and \ssd\ respectively).

%In contrast, with bigger I/O size (> 4KB), \daxio\ has very almost the same break-even interval as the \fileio\ in \fsdax\ and \sector\ mode which is due to their close throughput as reported in Section \ref{sec: micro_res}. Besides, those break-even interval values of \nvm\ are larger than that of \ssd. The reason is that although \nvm\ has at least 4x better throughput than \ssd\ with larger I/O size, \ssd\ has much smaller \textit{economic ratio} than \nvm\ (\$0.22/GB VS \$6.25/GB), outweighing the throughput benefit of \nvm.
% This is because different configurations over \nvm\ share the same {\em economic ratio} and thus the break-even interval values should only depend on the throughput values, which again justifies the effectiveness of \daxio\ in \nvm.

%Second, as expected, the more expensive the \nvm\ is, the larger the break-even value will be for \daxio\ and \fileio\ over \nvm, which is even larger than that of \ssd\ when the unit price is \$10/GB and the I/O size is over 4 KB (the gray bar in Figure \ref{fig:five-min_rr_10} is lower than other bars). But even when unit price is as high as \$10/GB, we can still see smaller break-even interval in \daxio\ in \fsdax\ mode compared to \ssd\ for small I/Os, i.e. 512 Bytes I/O size. 

%To further explore in which price range, \daxio\ in \fsdax\ mode has smaller break-even interval values compared to \ssd, we present how the break-even interval values change with the varied \nvm\ unit price with two different I/O sizes, i.e. 512 Bytes and 8 KB in Figure \ref{fig:five-min_rr_price_change_512b} and \ref{fig:five-min_rr_price_change_8k} respectively. 

%As Figure \ref{fig:five-min_rr_price_change_512b} shows, with small I/O size, when the unit price of \nvm\ is smaller than \$29.75/GB, \nvm\ is better, which, however, is far larger than the unit price of DRAM. Since we expect that the stable unit price of \nvm\ should lie between that of DRAM and that of \ssd, we should expect that \nvm\ should be always better in break-even interval values with small I/O size. In contrast, with larger I/O size (see Figure \ref{fig:five-min_rr_price_change_8k}), the unit price threshold is smaller than that of DRAM (\$3.63/GB VS \$6.25/GB), indicating that we should avoid using \daxio\ with larger I/O sizes.






\cmt{for fair comparison, we should also discuss about SSDs with 512 GB. Enterprise SSDs VS regular SSDs}


%\textbf{Discussions:} Although the evaluations of break-even interval above are based on the performance measurements over \nvm\ with 2DIMMs, i.e. 2 \nvm s, the  break-even interval value does not depend on the number of DIMMs. This is because in Equation \ref{eq: five-min-rule}, changing the number of DIMMs results in the same scaling over $PricePerDiskDrive$ and IOPS, i.e. $AccessPerSecondPerDisk$ term, thus eliminating the effect of multiple identical devices in the system. 

%However, it is still far away for fair comparisons between \nvm\ and \ssd. The reason is that the throughput of \ssd\ depends on the number of lanes and thus \ssd\ with smaller size has the same throughput but cheaper price, which means that smaller break-even interval is expected if the size of \ssd\ is also reduced to 512 GB and the unit price keeps the same. So we listed all the available 512GB SSDs and their potential price range in Table \ref{table: nvme_ssd_512}.  since the size of \ssd\ is larger than that of \nvm\ while smaller size of \ssd\ can deliver almost the same bandwidth, which  So the evaluation above can be a fair comparison between \nvm\ can \ssd.

%In contrast, when \nvm\ is configured as memory mode, opposite patterns appear with increasing \nvm\ unit price, i.e. the break-even interval values become smaller. When the unit price of \nvm\ is higher than that of DRAM (\$10/GB VS \$6.5/GB), the corresponding break-even interval values are smaller than that of \ssd\ with DRAM as the memory. It indicates that when \nvm\ is more expensive than DRAM, the better choice is to configure \nvm\ as memory mode and use \ssd\ as persistent storage, which not only provide memory with large capacity but also save memory usage compared to DRAM-\ssd\ configuration. Furthermore, by analysis above and results in Table \ref{table: price-threshold}, we can find that in some cases, e.g. when I/O size is 512 Bytes or 1 KB, \nvm\ should be always selected by configuring it either as memory mode or fsdax mode using \daxio. For other I/O sizes such as 4KB, the use of \ssd\ without using \nvm\ can save memory usage only when the unit price of \nvm\ lies in [4.03, 6.5] (for random read I/O) or [4.60, 6.5] (for sequential read I/O), which, however, is a quite small price range.



%Let's assume that a table $R$ has $n$ records in total, which is also attached with B-tree index. Suppose each record in the index page consumes 30 bytes on average, each page reserves 20 bytes for its header and the I/O size is $B$, then the number of the pointers in each intermediate node will be $\frac{B-20}{30}$ and the total number of index pages in the leaf nodes for the $n$ records will be $\frac{n}{(B-20)/30}$. So the height of this B-tree is $log_{\frac{B-20}{30}}(\frac{n}{(B-20)/30})$. If the I/O time to retrieve some specific index page is $t$, then the total I/O time to retrieve a specific index record will be $t \times log_{\frac{B-20}{30}}(\frac{n}{(B-20)/30})$. Then we can apply the latency values that we got from the microbenchmark results to compute the overhead of B-tree index search with varied I/O size and configurations, which are presented in Table \ref{table: index-overhead} (suppose $n = 10^6$).

%As Table \ref{table: index-overhead} shows, for \fileio\ over either \nvm\ or \ssd, the minimal indexing access latency appears when the I/O size is relatively large (4KB for \nvm\ \fileio\ in both fsdax and sector modes while 16KB for \ssd). In contrast, the corresponding I/O size is 256 Bytes or 512 Bytes for \daxio\ in fsdax mode, which is around 7x faster than \fileio\ over \nvm\ and two orders of magnitude faster than \ssd, which, again, indicates the performance advantages of \nvm\ \daxio\ with small I/O sizes. It means that in order to fully maximize the performance gains from \daxio\ in B-tree involved queries, we should consider transform the B-tree index I/O size to 256 Bytes or 512 Bytes.



%\begin{table*}[h]
%\centering
%\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}\hline
%I/O size&64B & 128B & 256 B&512 B & 1KB & 2KB & 4KB & 8KB& 16KB & 32KB& 64KB\\\hline
%\makecell{\nvm\ fsdax \daxio} &3.86&1.57&0.97&0.98&1.41&1.69&2.03&3.03&4.78&8.33&13.46\\\hline
%\makecell{\nvm\ fsdax \fileio}\ & 81.72&23.78&13.79&9.97&8.45&7.47&6.78&7.44&9.41&13.36&20.24
%\\ \hline
%\makecell{\nvm\ sector \fileio} &-&-&-&-&-&-&7.54&8.30&10.74&16.50&21.53\\ \hline
%\makecell{\ssd\ \fileio} &-&-&-&309.79&235.63&187.02&147.91&140.47&139.76&156.98&168.38\\ \hline
%%\makecell{\nvm\ -\ssd}&-&341.82&239.62&189.96&154.11&135.29&134.71&146.03&168.37\\\hline
%\end{tabular}
%\caption{Index access overhead ($\mu$s)}\label{table: index-overhead}
%\end{table*}
\cmt{optional: B-tree index implementation discussions, software overhead and caching effect}
%
%some theoretical analysis for some typical queries, e.g. sequential scan, aggregate queries, join queries, sort queries
%+
%some results from synthetic database workload and standard database workload
%
%
%
%
%\cmt{
%compare the break-even values in different modes. Talk about insights by combining the microbenchmark results.
%
%possible conclusion: due to the better IO performance of pmem in fsdax mode, its break-even value is smaller and thus we do not have to cache data in the memory for long time, which helps save memory.}


\subsection{\nvm\ as memory}\label{sec: perf_cost_mem}

Consider the in-memory database with workset data larger than typical DRAM capacity (e.g. 2 TB, which has been studied in some earlier works on main-memory database \cite{ma2016larger}), to finish certain workload over this workset, it will take about $2TB /(20GB/s) = 100 s$ and the total price of \nvm\ is $\$ 6.25/GB \times 2TB = \$ 12500 $



\cmt{note that we should talk about the sharp increase of the DRAM price when the memory capacity doubles}

In contrast, to finish the same operations over the same amount of workset data (2 TB) within the same amount of time (100 s), not all the hot data should be put in DRAM. So the performance bottleneck will be the overhead to load the data from SSD to DRAM. Considering the fact that the maximal read bandwidth of \ssd\ is around 3GB/s, then to make sure that the memory operations can be done within 100 s, the maximal amount of hot data to be put in \ssd\ should be $3GB/s * 100s = 300GB$ and thus the rest of the hot data should be cached in DRAM, which needs $2TB-300GB = 1.7TB $ DRAM in total. We can assume that we still use the same machine with the same number of memory slots (12 DRAM DIMM). To hold 1.7 TB  DRAM, each DRAM slot should be around 140 GB. According to the price information from \footnote{https://memory.net/memory-prices/}, the price of each 128GB DRAM is at least \$ 1400, which means that the total cost on 1.7TB DRAM should be at least $\$ 16800$. Compared to current configuration where we have $12\times 16GB$ DRAM, the extra cost on DRAM will be $\$ 16800 - \$ 6.25/GB \times 16GB = \$15575 $, which is more expensive than using \nvm\ as memory.




%Doing some analysis for performance VS price trade-offs (similar to the five-minute rule): after obtaining some charts to show the relative performance between \mmdram\ and \mmcache, to obtain the same throughput as \mmcache\ when the dataset is large enough, we can approximately calculate how many extra DRAMs that we need to purchase. Ideally, the \mmcache\ should help us save money based on the calculations.







==> Sections/research_direction.tex <==
\section{Future research direction with \nvm}\label{sec: future-work}
%First of all,
As we have seen, \nvm\ has extremely low latency and higher throughput compared to SSDs, enabling it to boost the performance in I/O intensive applications.
For example, we should expect better I/O performance in database systems once \nvm\ is used in the storage layer. \bpk{but our results suggest that that additional work is required here ... this section should enumerate what that is}
There also exists other potential uses for \nvm, such as scalable deep learning, in which the I/O becomes the major overhead as \cite{pumma2019scalable} mentioned.

One of the most outstanding performance characteristics of \nvm\ is its performance gains with small random reads using \daxio\, suggesting its potential in random index accesses in database systems.
According to our theoretical analysis in Section  \ref{sec: b-tree}, the optimal index page size by using \daxio\ should be 512 Bytes, which can alleviate the waste of I/O bandwidth when there is only small portions of the index pages required by some workloads.
Plus, 512 Bytes is closer to CPU cache-line size compared to traditional database page sizes.
So it is worth revisiting some of the prior work on B-tree index design by taking into consideration the CPU cache effect \cite{hankins2003effect}.
\bpk{or probably even evaluating more traditional in-memory structures (e.g. BW-Tree, order preserving hash-tables, etc.) for larger cache-line sized tuning}
% As \cite{chien2018characterizing} indicates, to hide the latency of loading training data from file system in current , the training samples used at each iteration are pre-fetched beforehand and cached in the buffer. So there is an opportunity to utilize \nvm\ to reduce I/O overhead without consuming the extra buffers.


\cmt{small random writes in file systems?}

